A Larson-Sweedler Theorem for Hopf V-Categories

The aim of this paper is to extend the classical Larson-Sweedler theorem, namely that a k-bialgebra has a non-singular integral (and in particular is Frobenius) if and only if it is a finite dimensional Hopf algebra, to the `many-object' setting of Hopf categories. To this end, we provide new characterizations of Frobenius V-categories and we develop the integral theory for Hopf V-categories. Our results apply to Hopf algebras in any braided monoidal category as a special case, and also relate to Turaev's Hopf group algebras and particular cases of weak and multiplier Hopf algebras.

==> tikzlibrarystrings.code.tex <==

%end of line command
\newcommand{\stringendline}{
\tikzset{shift={(-\currentwidth,-1)}};
\tikzmath{\currentwidth=0.0;}
}
%pad line with empty space of specified length
\newcommand{\pad}[1]{
\tikzset{shift={(#1,0)}}
\tikzmath{\currentwidth = \currentwidth + #1;} 
}
%pad line with empty space of length 1
\newcommand{\zero}{\pad{1}}
%a single vertical line
\newcommand{\one}{
\draw [very thick, line cap=round] (0, 0) -- (0,-1);
\tikzset{shift={(1,0)}}
\tikzmath{\currentwidth = \currentwidth+1;} 
}
%a single line stretching to the left #1 units
\newcommand{\lone}[1]{
\draw [very thick, line cap=round] (0, 0) -- (-#1,-1);
\tikzset{shift={(#1+1,0)}}
\tikzmath{\currentwidth = \currentwidth+#1+1;} 
}
%a single line stretching to the right #1 units
\newcommand{\rone}[1]{
\draw [very thick, line cap=round] (0, 0) -- (#1,-1);
\tikzset{shift={(#1+1,0)}}
\tikzmath{\currentwidth = \currentwidth+#1+1;} 
}
%a left-to-right crossing of width 2*#1
\newcommand{\Braid}[1][1.0]{
\draw [very thick, line cap=round] (#1, 0) -- (0,-1);
\draw [white, line width=6] (.2*#1, -.2) -- (.8*#1,-.8);
\draw [very thick, line cap=round] (0, 0) -- (#1,-1); 
\tikzset{shift={(2*#1,0)}}
\tikzmath{\currentwidth = \currentwidth+2*#1;} 
}
\newcommand{\oBraid}{
\draw [very thick, line cap=round] (1,0) .. controls (1,-.5)  and (0,-.5) .. (0,-1);
\draw [white, line width=6] (.3, -.4) -- (.7,-.6);
\draw [very thick, line cap=round] (0,0) .. controls (0,-.5)  and (1,-.5) .. (1,-1);
\tikzset{shift={(2,0)}}
\tikzmath{\currentwidth = \currentwidth+2;} 
}

%a right-to-left crossing of width 2*#1
\newcommand{\rBraid}{
\draw [very thick, line cap=round] (0, 0) -- (1,-1); 
\draw [white, line width=6] (.8, -.2) -- (.2,-.8);
\draw [very thick, line cap=round] (1, 0) -- (0,-1);
\tikzset{shift={(2,0)}}
\tikzmath{\currentwidth = \currentwidth+2;} 
}

%a left-to-right crossing of width #1+1
\newcommand{\nBraid}[1]{
\foreach \x in {1,...,#1}
{
	\draw [very thick, line cap=round] (\x, 0) -- (\x - 1, -1);
}
\draw [white, line width=6] (0.1*#1, -.1) -- (0.9*#1,-.9);
\draw [very thick, line cap=round] (0, 0) -- (#1,-1); 
\tikzset{shift={(#1+1,0)}}
\tikzmath{\currentwidth = \currentwidth+#1+1;} 
}

%a cup of width 2
\newcommand{\cuppp}{
\draw [very thick] (0,0) arc (180:360:.5);
\tikzset{shift={(2,0)}}
\tikzmath{\currentwidth = \currentwidth+2;} 
}

%a cap of width 2
\newcommand{\cappp}{
\draw [very thick] (0,-1) arc (180:0:.5);
\tikzset{shift={(2,0)}}
\tikzmath{\currentwidth = \currentwidth+2;} 
}

\newcommand{\counit}{
\draw [very thick, line cap=round] (0, 0) -- (0,-.5);
\draw [fill=white] (0,-.5) circle (0.1);
\tikzset{shift={(1,0)}}
\tikzmath{\currentwidth = \currentwidth+1;} 
}
\newcommand{\Atpd}{
\draw [very thick, line cap=round] (0, 0) -- (0,-1);
\draw [fill=white] (0,-.5) circle (0.1);
\tikzset{shift={(1,0)}}
\tikzmath{\currentwidth = \currentwidth+1;} 
}
\newcommand{\mult}{
\draw [very thick, line cap=round] (0, 0) -- (.5,-.5);
\draw [very thick, line cap=round] (1, 0) -- (.5,-.5);
\draw [very thick, line cap=round] (.5, -.5) -- (.5,-1);
\tikzset{shift={(2,0)}}
\tikzmath{\currentwidth = \currentwidth+2;} 
}
\newcommand{\omult}{
\draw [very thick] (0,0) arc (180:360:.5);
\draw [very thick, line cap=round] (.5, -.5) -- (.5,-1);
\tikzset{shift={(1,0)}}
\tikzmath{\currentwidth = \currentwidth+1;} 
}
\newcommand{\comult}{
\draw [very thick, line cap=round] (0, -1) -- (.5,-.5);
\draw [very thick, line cap=round] (1, -1) -- (.5,-.5);
\draw [very thick, line cap=round] (.5, -.5) -- (.5,0);
\tikzset{shift={(1,0)}}
\tikzmath{\currentwidth = \currentwidth+1;} 
}
\newcommand{\ocomult}{
\draw [very thick] (0,-1) arc (180:0:.5);
\draw [very thick, line cap=round] (.5, -.5) -- (.5,0);
\tikzset{shift={(2,0)}};
\tikzmath{\currentwidth = \currentwidth + 2;} 
}

\newenvironment{tikzstrings}
    {
    \begin{tikzpicture}
    \tikzmath{
	\currentwidth = 0.0;}
	\begingroup
	\def\1{\one}
	\def\0{\zero}
	\def\\{\stringendline}
    }
    { 
    \endgroup
    \end{tikzpicture}
    }

    
